Fence Synthesis under the C11 Memory Model

The C/C++11 (C11) standard offers a spectrum of ordering guarantees on memory access operations. The combinations of such orderings pose a challenge in developing correct and efficient weak memory programs. A common solution to preclude those program outcomes that violate the correctness specification is using C11 synchronization-fences, which establish ordering on program events. The challenge is in choosing a combination of fences that (i) restores the correctness of the input program, with (ii) as little impact on efficiency as possible (i.e., the smallest set of weakest fences). This problem is the optimal fence synthesis problem and is NP-hard for straight-line programs. In this work, we propose the first fence synthesis technique for C11 programs called FenSying and show its optimality. We additionally propose a near-optimal efficient alternative called fFenSying. We prove the optimality of FenSying and the soundness of fFenSying and present an implementation of both techniques. Finally, we contrast the performance of the two techniques and empirically demonstrate fFenSyings effectiveness.

==> proofs/optimality_sketch.tex <==
(i) \wkfence and \stfence are sound 
$\implies$
\sat query has every possible cycle
$\implies$
{\tt min}$\Phi$ returns a smallest cycle (assuming \sat solver is sound).
%
(ii) Each fence is locally assigned the weakest memory order ($m$)
(by design of {\tt assignMO}).
%
(iii) If global memory order ($m' \mogt m$) then a cycle has the same
fence with memory order $m'$
$\implies$
$m$ is not globally sound.
%
Refer Appendix~\ref{adx:proofs} for formal proof by induction on $|${\tt BT}$|$.

==> proofs/soundness_sketch.tex <==
\ourtechnique is sound for $|${\tt BT}$|$ = 1 (same argument as 
Theorem~\ref{pthm:fastfensying sound}).
%
Given $|${\tt BT}$|$ = N.
%
(i) \sat query retains at least 1 cycle per trace (by construction).
%
(ii) Final memory order are not weaker than those assigned initially by
{\tt asignMO}.
%
Hence proved by induction on $|${\tt BT}$|$.
Refer Appendix~\ref{adx:proofs} for formal proof.

==> proofs/soundness_sketch_fast.tex <==
(i) \wkfence and \stfence are sound 
(Lemmas~\ref{lem:weak-sound},\ref{lem:strong-sound});
%
(ii)
At least 1 candidate solution is in {\tt min}$\Phi$ (by construction);
%
(iii)
Fence memory order are sufficiently strong (Lemma~\ref{lem:mo-sound}).
%
Refer Appendix~\ref{adx:proofs} for formal proof.

==> sections/implementation.tex <==
The techniques have been implemented in {\tt Python}.
\wkfence and \stfence uses {\em Johnson's} cycle detection algorithm 
available in the {\em networkx} library.
%
We use \z theorem prover to find the {\em min-model} of \sat 
queries.
We recognized \cds \cite{cds} as the closest match to the
specification of a buggy trace generator
for the following reasons;
%
\begin{enumerate}
	\item \cds supports the \cc semantics. Most other techniques are
	designed for a variant \cite{genmc-PLDI19} or subset
	\cite{abdulla2019verification,tracer2018} of \cc.
	
	\item \cds is a stateless model checker that returns buggy traces 
		along with the corresponding $\setHB$, $\setRF$ and $\setMO$ relations.
	
	\item \cds does not halt at the detection of the first buggy 
		trace instead it continues to provide all buggy traces as 
		required by \ourtechnique.
		
	\item \cds is open-source.
\end{enumerate}
%
To bridge the gap between \cds's output and our requirements,
we modify \cds's code to accept program location as an attribute of the 
program events and to halt at the first buggy trace when specified.



\noindent
{\bf Time efficient alternative technique (fasttechnique):} 
It was observed that 
analysis time of the core technique and \z computation of min-model 
were impacted by the number of buggy traces returned by \cds.
%
It was also observed that typically a set of synthesized fences 
can invalidate multiple buggy traces.
%
On the above observations we propose a time efficient alternative 
to the core technique that considers one buggy trace at a time
called fasttechnique.
%
fasttechnique picks any one buggy trace $\tau$ of $P$,
fixes $\tau$ and transforms $P$ to $P'$,
where $P'$ contains the newly added fences along with the events 
originally in $P$. 
%
The technique then looks for the next buggy trace by invoking \cds 
with $P'$ as the input program. 
The process repeats till \cds returns no buggy traces, or
finds a buggy trace that cannot be fixed with \cc fences.
%
%\begin{wrapfigure}{r}{0.55\columnwidth}
%	\small
%	\begin{tabular}{|l|}
%		\multicolumn{1}{r}{\scriptsize $e_i$: program events,
%			$\mathbb{F}_i$: candidate fences} \\
%		
%		\hline
%		cycles in $\tau_1$ (${\tt C}_{\tau_1}$): \\
%		\tab $\{\mathbb{F}_1, \mathbb{F}_2, e_1\}$ and
%		     $\{\mathbb{F}_1, \mathbb{F}_3, \mathbb{F}_4\}$\\
%		$\formula{{\tt C}_{\tau_1}}$ = ($\mathbb{F}_1 \^ \mathbb{F}_2$) $\v$ ($\mathbb{F}_1 \^ \mathbb{F}_3 \^ \mathbb{F}_4$)\\
%		\\
%		cycles in $\tau_2$ (${\tt C}_{\tau_2}$):
%		$\{\mathbb{F}_3, \mathbb{F}_4\}$\\
%		$\formula{{\tt C}_{\tau_2}}$ = ($\mathbb{F}_3 \^ \mathbb{F}_4$)\\
%		\hline
%				
%		\multicolumn{1}{c}{\footnotesize\hl{3-fence}}
%	\end{tabular}
%\end{wrapfigure}
%
The technique is sound, \ie if $P$ can be fixed with \cc fences 
then fasttechnique will successfully fix $P$;
but the technique is not optimal.
The nonoptimality of fasttechnique is a result of the reduction 
in information that the technique has to work with (from all 
buggy traces to just one at a time). As a consequence of considering one 
trace per iteration the \z formula is attenuated with terms only from 
one trace.
%
Consider the example in Figure~\hlref{3-fence} 
depicting cycles in two buggy traces $\tau_1$ and $\tau_2$ of an 
input program, where $\mathbb{F}_i$ for $i \in [1,4]$ represents 
candidate fences and $e_1$ represents a program event.
The optimal \ourtechnique 
technique would provide the formula $\formula{{\tt C}_{\tau_1}}$ $\^$ 
$\formula{{\tt C}_{\tau_2}}$ to \z and thus recognize ($\mathbb{F}_1 \^ 
\mathbb{F}_3 \^ \mathbb{F}_4$) as the optimal solution.
fasttechnique, however, may consider the formula 
$\formula{{\tt C}_{\tau_1}}$ in the first iteration and 
$\formula{{\tt C}_{\tau_2}}$ in the next iteration and return
($\mathbb{F}_1 \^ \mathbb{F}_2$) $\^$ ($\mathbb{F}_3 \^ \mathbb{F}_4$) 
as the result which is not optimal in the number of fences.
%
However, it was observed from the experimental results that the time
efficient technique significantly outperforms the optimal technique in 
terms of the analysis time while adding a reasonably small number of 
extra fences. The experimental results have been discussed in 
$\mathsection$\ref{sec:results}.
